Constrained Dynamic Movement Primitives for Safe Learning of Motor Skills

Dynamic movement primitives are widely used for learning skills which can be demonstrated to a robot by a skilled human or controller. While their generalization capabilities and simple formulation make them very appealing to use, they possess no strong guarantees to satisfy operational safety constraints for a task. In this paper, we present constrained dynamic movement primitives (CDMP) which can allow for constraint satisfaction in the robot workspace. We present a formulation of a non-linear optimization to perturb the DMP forcing weights regressed by locally-weighted regression to admit a Zeroing Barrier Function (ZBF), which certifies workspace constraint satisfaction. We demonstrate the proposed CDMP under different constraints on the end-effector movement such as obstacle avoidance and workspace constraints on a physical robot. A video showing the implementation of the proposed algorithm using different manipulators in different environments could be found here https://youtu.be/hJegJJkJfys.

==> introduction.tex <==
\section{Introduction}\label{sec:intro}
Learning from Demonstration (LfD) is a powerful technique that allows 
Dynamic Movement Primitives (DMPs) are a nonlinear dynamical system formulation that can learn complex trajectories from demonstrations by decoupling a nonlinear forcing function from the nominal attraction behavior. These systems can be re-parameterized by their start and goal positions, but direct control over executed trajectory in between these poses is very difficult. Without care, a new start or goal pose may cause the robot to collide with itself or the environment or extend past its own joint limits.

We present Constrained DMPs, which constrains the end-effector to stay within a tube where the robot is known to be free of link collisions and joint-limit extensions. 
